MT-CGCNN: Integrating Crystal Graph Convolutional Neural Network with Multitask Learning for Material Property Prediction

Developing accurate, transferable and computationally inexpensive machine learning models can rapidly accelerate the discovery and development of new materials. Some of the major challenges involved in developing such models are, (i) limited availability of materials data as compared to other fields, (ii) lack of universal descriptor of materials to predict its various properties. The limited availability of materials data can be addressed through transfer learning, while the generic representation was recently addressed by Xie and Grossman [1], where they developed a crystal graph convolutional neural network (CGCNN) that provides a unified representation of crystals. In this work, we develop a new model (MT-CGCNN) by integrating CGCNN with transfer learning based on multi-task (MT) learning. We demonstrate the effectiveness of MT-CGCNN by simultaneous prediction of various material properties such as Formation Energy, Band Gap and Fermi Energy for a wide range of inorganic crystals (46774 materials). MT-CGCNN is able to reduce the test error when employed on correlated properties by upto 8%. The model prediction has lower test error compared to CGCNN, even when the training data is reduced by 10%. We also demonstrate our model's better performance through prediction of end user scenario related to metal/non-metal classification. These results encourage further development of machine learning approaches which leverage multi-task learning to address the aforementioned challenges in the discovery of new materials. We make MT-CGCNN's source code available to encourage reproducible research.

==> sections/related.tex <==
\section{Related work}
\label{sec:related_work}

\textbf{Graph neural networks}: {\it Geometric deep learning} \citep{gdl17} is an umbrella phrase for emerging techniques attempting to generalise (structured) deep neural network models to non-Euclidean domains such as graphs and manifolds. 

The earliest attempts to generalise neural networks to graphs use recurrent neural networks (RNN) to learn representations for classification or regression of nodes or graphs \citep{gnn05,gnn09}.
{\color{red} Subsequently, a CNN-like deep neural architecture on graphs was formulated in a pioneering work by giving a mathematically sound definition of the convolution operation on graph signals in the {\it spectral domain} \citep{gcn_iclr14}.
A second formulation of convolution on graph is in the {\it spatial domain} in which the localisation property of convolution is provided by construction \citep{gcn_iclr14}.}
One of the first formulations of a spatial CNN-like neural network on graph generalised standard molecular feature extraction methods based on circular fingerprints \citep{DuvenaudMAGHAA15,gcn_camd16}. This architecture has also been employed for few shot learning to learn distance metrics in drug discovery applications \citep{lddd_acs17}. Recently, all of the above types (RNN, spectral CNN, spatial CNN on graph) have been unified into a single message passing neural network (MPNN) framework \citep{mpnn_icml17} and a variant of MPNN has been shown to achieve state-of-the-art results on an important molecular property prediction benchmark.
Crystal graph convolutional neural networks \citep{CGCNN} have been developed for predicting useful material properties directly through graphs constructed from the connections of atoms in crystals.

\textbf{Multi-task learning}: Multitask learning (MTL) is the procedure of learning several tasks at the same time with the objective of mutually benefitting the performance of individual tasks. This concept has been applied to various domains. Good overview of the various aspects of multi-tasking could be found in \citep{Caruana1997, Ruder17a}. Using multi-task learning has shown improvements in various fields of machine learning, from natural language processing \citep{Collobert08}, computer vision \citep{Girshick15} to drug discovery \citep{Ramsundar15} and pharma \citep{Ramsundar17}.
Also, there has been some recent work on using multi-tasking with graph neural networks (GNNs). It has been shown that techniques for matrix completion in recommender systems can be improved by exploiting user-user and item-item relationships in a multi-task manner \citep{mgcnn_nips17}. Learning to multitask \citep{l2mt_nips18} uses a GNN to exploit historical multitask experience to learn how to choose a suitable multitask model for a new mutitask problem.
Along with the various applications of multi-task learning, good progress has been made towards building systematic approaches to perform multi-tasking. In \citep{KendallGC17, Gradnorm17}, the authors explore how weight coefficients can be learnt for a weighted loss approach to MTL. Recently, multi-tasking has been framed as a multi-objective optimization problem \citep{Sener18}.
